Omitting continuous covariates in binary regression models: implications for sensitivity and mediation analysis

By exploiting the theory of skew-symmetric distributions, we generalise existing results in sensitivity analysis by providing the analytic expression of the bias induced by marginalization over an unobserved continuous confounder in a logistic regression model. The expression is approximated and mimics Cochran's formula under some simplifying assumptions. Other link functions and error distributions are also considered. A simulation study is performed to assess its properties. The derivations can also be applied in causal mediation analysis, thereby enlarging the number of circumstances where simple parametric formulations can be used to evaluate causal direct and indirect effects. Standard errors of the causal effect estimators are provided via the first-order Delta method. Simulations show that our proposed estimators perform equally well as others based on numerical methods and that the additional interpretability of the explicit formulas does not compromise their precision. The new estimator has been applied to measure the effect of humidity on upper airways diseases mediated by the presence of common aeroallergens in the air.

==> simulation.tex <==
\section{Simulation study}
\label{sec:simulation}
We carried out a simulation study in order to invastigate the performance of our proposed estimators for the natural effects and to compare it with the existing ones. Parameters are chosen  as in \textcite{samoilenko2022}, as follows. The variable $X$ and the mediator $W$ were simulated respectively from a $Bern(p_x)$, and a $\mathcal{N}(\theta_0 + \theta_x x, \sigma^2)$ with $p_x=0.3$, $\theta_0=0.1$, $\theta_x=0.5$ and $\sigma=0.5$. While, the response was simulated from a $Bern(p_y)$, where $\log(p_y/(1-p_y))=\beta_0 + \beta_x x + \beta_w w + \beta_{xw} xw$, with $\beta_x=0.4$, $\beta_w=0.5$, $\beta_{xw}=0.15$ and $p_y$ denoting $\pr(Y=1 \mid X=x, W=w)$. In order to obtain different percentages of rareness for our response we varied the intercept of the logistic regression $\beta_0=\{-3, -2, -0.5, 1, 2\}$, choosing these specific values for the intercept the marginal prevalences are 6.65\%, 15.95\%, 44.52\%, 77.23\% and 90.03\%. In addition, every simulation is performed with 4 different sample sizes $n=\{150, 500, 1000, 5000\}$ to take into account the adequacy of the methods in different scenarios. 

The proposed methods was compared to the methods described in \textcite{vander2013} (VV), \textcite{gaynor2018} (Gaynor), \textcite{samoilenko2022} (Exact) and to the NEM approach \parencite{lange2012} (Nem). For each simulation we generated 1000 independent samples and we reported, for every combination of $\beta_0$ and $n$, the bias and the standard deviation. The true value of each scenario was computed via numeric integration based on \texttt{QUADPACK} \parencite{piessens2012}. For our method we calculated the coverage of the 95\% confidence intervals obtained via Delta method (see Appendix \ref{appendix_b}), while for NEM approach the coverage of the 95\% confidence intervals was constructed using SEs based on sandwich estimator. For all methods except NEM, 95\% confidence intervals based on percentile bootstrap with 500 replication were reported. The results for the NEM approach were obtained using the imputation approach implemented in the R package \texttt{medflex} \parencite{steen2017}.

In Table \ref{tab:nde}, the performance of the various estimators of the NDE is presented. In terms of bias,  our proposed estimator performs as well as the exact and the NEM methods, and the three outperforms the others, with the only exception of VV, that in the $\beta_0=-3$ and $\beta_0=-2$ also performs well (and it is actually the best for $n=150$). Gaynor's approach performs well only the outcome is common, in line with other simulation studies, such for example \textcite{cheng2021estimating}. Similar considerations apply to the empirical coverage of the 95$\%$ confidence interval, where, however, for small sample size, for our proposed method the empirical coverage is better for confidence intervals based on the delta methods rather than on bootstrap (with the exception of a balanced outcome, a case in which they both perform well).  Analogous considerations apply to the performance of the estimators of the NIE, see Table \ref{tab:nie}. In line with the literature based on the continuous-continuos case, see for example \textcite{mackinnon2004confidence, biesanz2010assessing}({\bf inserire quotation cercare?}), the empirical coverage of confidence intervals for NIE is good only for very large sample sizes for all methods. 

Overall, inspection of the two tables shows that the method here proposed presents satisfactory results for all configurations, unlike other methods that work well only under particular conditions of the binary response, such as rareness or commonness, such as the approaches in \textcite{vander2013} or \textcite{gaynor2018}. In particular, it seems to offer comparable accuracy with the NEM approach and the exact regression-based method for both direct and indirect effects that, however, provide no parametric intuition of the results. A large error, due to the sparse-data bias, appears for $n=150$ in all the methods presented. A possible solution is the use of Firth's correction \parencite{firth1993} to reduce the bias of the Maximum Likelihood estimates, as proposed in \textcite{samoilenko2022}. The coverage of the CIs obtained via Delta method is adequate for all sample size bigger than 500 and for all values of $\beta_0$, and in general it is better for NDE. 

A proper coverage of percentile bootstrap is obtained for sample sizes bigger than 150 if our method is used,

To summarise, the precision of our proposed estimators is better than or at least comparable with the others for all levels of rareness/commonness of the outcome. In addition, bias is negligible for all $n$ and it decreases with increasing the sample size, while standard errors are the smallest in many of the proposed configurations. Our estimators performs as well as other based on numerical methods, with the additional benefit of a allowing the interpretation of the effects, as functions of the parameters of the data-generating process.
